Guided Co-Modulated GAN for 360{\deg} Field of View Extrapolation

We propose a method to extrapolate a 360{\deg} field of view from a single image that allows for user-controlled synthesis of the out-painted content. To do so, we propose improvements to an existing GAN-based in-painting architecture for out-painting panoramic image representation. Our method obtains state-of-the-art results and outperforms previous methods on standard image quality metrics. To allow controlled synthesis of out-painting, we introduce a novel guided co-modulation framework, which drives the image generation process with a common pretrained discriminative model. Doing so maintains the high visual quality of generated panoramas while enabling user-controlled semantic content in the extrapolated field of view. We demonstrate the state-of-the-art results of our method on field of view extrapolation both qualitatively and quantitatively, providing thorough analysis of our novel editing capabilities. Finally, we demonstrate that our approach benefits the photorealistic virtual insertion of highly glossy objects in photographs.

==> 3_imageformation.tex <==
\section{Image formation model}
\label{sec:image-formation}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/image_formation.pdf}
  \caption{When a camera takes a picture (inset right), it samples a part of the environment around it, which can be represented in 2D as a latitude-longitude 360\degree{} panorama image (top).}
  \label{fig:image-formation}
\end{figure}

As is commonly done in the literature~\cite{Hara_Mukuta_Harada_2021,akimoto2019360,somanath2021hdr}, we frame $360^\circ$ field of view extrapolation as out-painting in a latitude-longitude (or equirectangular) panoramic representation. We therefore warp the input image  $\mathbf{x}$ to a equirectangular representation according to a simplified camera model, \ie, 
%
\begin{equation}
\mathbf{p}_\mathrm{im} = \mathbf{K}\mathbf{R}\mathbf{p}_\mathrm{w} \,.
\label{eq:formation}
\end{equation}%
%
Here, $\mathbf{p}_\mathrm{w}$ represents a 3D point in world coordinates (whose origin coincides with the center of projection of the camera, hence no translation), and $\mathbf{p}_\mathrm{im}$ its projection (in homogeneous coordinates) on the image plane. We employ the pinhole camera model with common assumptions (principal point is the image center, negligible skew, unit pixel aspect ratio~\cite{Hartley2004}), hence $\mathbf{K} = \mathrm{diag}([f \; f \; 1])$, where $f$ is the focal length in pixels. 
%Instead of $f$, we use the vertical field of view $h_\theta = 2\arctan(\nicefrac{h}{2f})$, where $h$ is the image height. 

The rotation matrix $\mathbf{R}$ can be parameterized by roll $\gamma$, pitch $\beta$, and yaw $\alpha$ angles. Since an arbitrary image possesses no natural reference frame to estimate $\alpha$, we set $\alpha=0$. We also take $\gamma=0$ as in \cite{Hara_Mukuta_Harada_2021,akimoto2019360,somanath2021hdr}, hence $\mathbf{R} = \mathbf{R}_x(\beta)$. \Cref{fig:image-formation} illustrates our image formation model. 

In this work, we assume the necessary camera parameters $f$ and $\beta$ to be known. Other works, \eg, \cite{hold2017perceptual,xian2019uprightnet} could be used to estimate them otherwise. 



==> fig_editingresult_short.tex <==
\begin{figure} [t!]
    \centering
    \scriptsize
    \renewcommand{\tabcolsep}{1pt}
    \newcommand{\mywidth}{0.2\linewidth}
    \resizebox{\linewidth}{!}{% take the[] entire width, but still find a good per-image width otherwise text gets compressed
    \begin{tabular}{cccccc}
    Image 
    & Image-conditioned
    & $\mapsto \text{sky}$
    & $\mapsto \text{snow field}$
    & $\mapsto \text{promenade}$
    & $\mapsto \text{lawn}$
    \\
    \includegraphics[width=\mywidth]{figs/editing/qual/139116_partial.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/139116_src_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/139116_sky_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/139116_snowfield_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/139116_promenade_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/139116_lawn_generated.png}
    \\
    \includegraphics[width=\mywidth]{figs/editing/qual/514478_partial.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/514478_src_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/514478_sky_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/514478_snowfield_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/514478_promenade_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/514478_lawn_generated.png}
    \\
    \includegraphics[width=\mywidth]{figs/editing/qual/581272_partial.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/581272_src_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/581272_sky_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/581272_snowfield_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/581272_promenade_generated.png}
    & \includegraphics[width=\mywidth]{figs/editing/qual/581272_lawn_generated.png}
    \\
    \end{tabular}}
    \caption{Qualitative editing results via our novel guided style co-modulation mechanism. From different input images (``Image''), an extrapolated panorama is first obtained by our network (``Image-conditioned''). A user then selects different target labels, which are used to determine the optimal vector $\mathbf{g}^*$  for style co-modulation.}
    \label{fig:qual-editing}
\end{figure}


==> fig_objectinsertion.tex <==
\begin{figure*}[t]
    \centering
    \scriptsize
    \renewcommand{\tabcolsep}{1pt}
    \newcommand{\myheight}{1.8cm}
    % \resizebox{\linewidth}{!}{% take the[] entire width, but still find a good per-image width otherwise text gets compressed
    \begin{tabular}{ccc}
    Input image 
    & Extrapolated panorama 
    & Inserted virtual objects 
    \\
    % \includegraphics[height=\myheight]{figs/object_insertion/129785_crop.jpg}
    % & \includegraphics[height=\myheight]{figs/object_insertion/129785_src_generated.png}
    % & \includegraphics[height=\myheight]{figs/object_insertion/129785_render.png} 
    % \\
    \includegraphics[height=\myheight]{figs/object_insertion/100588_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/100588_src_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/100588_render.png} 
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/108254_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/108254_src_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/108254_render.png} 
    \\
    % \includegraphics[height=\myheight]{figs/object_insertion/129412_crop.jpg}
    % & \includegraphics[height=\myheight]{figs/object_insertion/129412_src_generated.png}
    % & \includegraphics[height=\myheight]{figs/object_insertion/129412_render.png} 
    % \\
    \end{tabular}
    \hspace{0.5em}
    \begin{tabular}{ccc}
    Input image 
    & Extrapolated panorama 
    & Inserted virtual objects 
    \\
    % \includegraphics[height=\myheight]{figs/object_insertion/286813_crop.jpg}
    % & \includegraphics[height=\myheight]{figs/object_insertion/286813_src_generated.png}
    % & \includegraphics[height=\myheight]{figs/object_insertion/286813_render.png} 
    % \\
    \includegraphics[height=\myheight]{figs/object_insertion/153703_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/153703_src_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/153703_render.png} 
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/128922_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/128922_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/128922_render.png} 
    \\
    \end{tabular}
    \begin{tabular}{ccc}
    Input image
    % & Extrapolated panoarama
    & Inserted virtual objects
    % & Edited panorama ($\mapsto \text{sky}$)
    & Inserted virtual objects
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/286813_crop.jpg}
    % & \includegraphics[height=\myheight]{figs/object_insertion/286813_src_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/286813_render.png} 
    % & \includegraphics[height=\myheight]{figs/object_insertion/286813_sky_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/286813_sky_render.png} 
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/129785_crop.jpg}
    % & \includegraphics[height=\myheight]{figs/object_insertion/129785_src_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/129785_render.png} 
    % & \includegraphics[height=\myheight]{figs/object_insertion/129785_courtyard_generated.png}
    & \includegraphics[height=\myheight]{figs/object_insertion/129785_courtyard_render.png} 
    \\
    \end{tabular}
    % }
    \caption{Virtual object insertion results. Our extrapolated panoramas can be used to realistically insert shiny virtual objects, which are particularly challenging in this context since they reflect the entire environment. By estimating a depth map from the panoramas and fitting a mesh to the output (see text), we can simulate spatially-varying reflections where appearance of the object changes as a function of its position in the scene. }
    \label{fig:object-insertion}
\end{figure*}


==> fig_objectionsertion-edit.tex <==
\begin{figure}[t]
    \centering
    \scriptsize
    \renewcommand{\tabcolsep}{1pt}
    \newcommand{\myheight}{1.7cm}
    \begin{tabular}{cccc}
    Input image
    & Image-conditioned
    & 
    & Edited
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/286813_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/286813_render.png} 
    & \rotatebox{90}{\scriptsize $\mapsto \text{``sky''}$} 
    & \includegraphics[height=\myheight]{figs/object_insertion/286813_sky_render.png} 
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/129785_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/129785_render.png} 
    & \rotatebox{90}{\scriptsize $\mapsto \text{``courtyard''}$} 
    & \includegraphics[height=\myheight]{figs/object_insertion/129785_courtyard_render.png} 
    \\
    \includegraphics[height=\myheight]{figs/object_insertion/153703_crop.jpg}
    & \includegraphics[height=\myheight]{figs/object_insertion/153703_render.png} 
    & \rotatebox{90}{\scriptsize $\mapsto \text{``beach''}$} 
    & \includegraphics[height=\myheight]{figs/object_insertion/153703_beach_render.png} 
    \\
    \end{tabular}
    \caption{With our guided co-modulation technique, a user can control the semantic content of the reflections on virtual objects, by generating more dramatic clouds ($\mapsto \text{``sky''}$), suggesting a more urban environment ($\mapsto \text{``courtyard''}$), and adding more sand to the surroundings ($\mapsto \text{``beach''}$). }
    \label{fig:object-insertion-edit}
\end{figure}

==> fig_qualresults.tex <==
\begin{figure}
    \centering
    \scriptsize
    \renewcommand{\tabcolsep}{1pt}
    \newcommand{\mywidth}{0.2\linewidth}
    \resizebox{\linewidth}{!}{% take the[] entire width, but still find a good per-image width otherwise text gets compressed
    \begin{tabular}{lcccccc}
    & Input 
    & Ground truth
    & pix2pixHD~\cite{wang2018high} 
    % & Symmetry~\cite{Hara_Mukuta_Harada_2021}-R 
    & Symmetry~\cite{Hara_Mukuta_Harada_2021}-G
    & \thename
    & Guided 
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 40^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/partial/19659_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/19659_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/40d/generated/19659_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/40d/rec/19659_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/40d/gen/19659_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/40d/generated/19659_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/generated/19659_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 40^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/partial/21967_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/21967_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/40d/generated/21967_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/40d/rec/21967_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/40d/gen/21967_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/40d/generated/21967_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/generated/21967_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 60^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/partial/180086_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/original/180086_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/60d/generated/180086_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/60d/rec/180086_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/60d/gen/180086_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/60d/generated/180086_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/generated/180086_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 60^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/partial/8582_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/original/8582_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/60d/generated/8582_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/60d/rec/8582_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/60d/gen/8582_0_partial_out_0.png} 
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/60d/generated/8582_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/60d/generated/8582_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 90^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/90d/partial/8008_0_full_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/90d/original/8008_0_full_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/90d/generated/8008_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/90d/rec/8008_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/90d/gen/8008_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/90d/generated/8008_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/90d/generated/8008_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 90^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/90d/partial/559576_0_full_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/559576_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/90d/generated/559576_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/90d/rec/559576_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/90d/gen/559576_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/90d/generated/559576_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/90d/generated/559576_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 120^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/partial/850107_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/original/850107_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/120d/generated/850107_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/120d/rec/850107_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/120d/gen/850107_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/120d/generated/850107_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/generated/850107_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 120^\circ$ \\ $\beta=0^\circ$}} 
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/partial/41272_0_full_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/original/41272_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/120d/generated/41272_0_full_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/120d/rec/41272_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/120d/gen/41272_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/120d/generated/41272_0_full_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/120d/generated/41272_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 44^\circ$ \\ $\beta=-8^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/782658_0_full_44_8_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/782658_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/782658_0_full_44_8_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/782658_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/782658_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/782658_0_full_44_8_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/782658_original_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 110^\circ$ \\ $\beta=23^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/744364_original_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/744364_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/744364_0_full_110_-23_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/744364_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/744364_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/744364_0_full_110_-23_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/744364_original_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 77^\circ$ \\ $\beta=-30^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/89000_0_full_77_30_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/89000_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/89000_0_full_77_30_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/89000_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/89000_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/89000_0_full_77_30_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/89000_original_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 92^\circ$ \\ $\beta=10^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/736147_0_full_92_-10_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/736147_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/736147_0_full_92_-10_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/736147_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/736147_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/736147_0_full_92_-10_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/736147_original_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 94^\circ$ \\ $\beta=-17^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/429560_0_full_94_17_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/429560_0_full_original.png} 
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/429560_0_full_94_17_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/429560_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/429560_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/429560_0_full_94_17_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/429560_original_generated.png}
    \\
    \rotatebox{90}{\parbox{1.3cm}{\centering $h_\theta = 97^\circ$ \\ $\beta=-4^\circ$}}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/partial/405479_0_full_97_4_partial.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/40d/original/405479_0_full_original.png}
    & \includegraphics[width=\mywidth]{figs/quant/pix2pixHD/random/generated/405479_0_full_97_4_0_synthesized_image.jpg}
    % & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/rec/405479_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/symmetry/random/gen/405479_0_partial_out_0.png}
    & \includegraphics[width=\mywidth]{figs/quant/CoModGAN++/random/generated/405479_0_full_97_4_generated.png}
    & \includegraphics[width=\mywidth]{figs/quant/ours/random/generated/405479_original_generated.png}
    \\
    \end{tabular}}
    \caption{Qualitative field of view extrapolation results. Previous works~\cite{wang2018high,Hara_Mukuta_Harada_2021} present obvious visual artifacts, including mode collapse in \cite{wang2018high} and blurriness for both. In contrast, our adaptations to CoModGAN enable high-quality extrapolation results (penultimate column), which are preserved by our novel guided co-modulation framework (last column). The first eight rows contain examples from the ``fixed-fov'' subset of our test set, while the last six are taken from the ``mixed'' subset. \textbf{See supplementary materials for more results}. }
    \label{fig:qual-comparison}
\end{figure}

